Hyperedge Prediction using Tensor Eigenvalue Decomposition

Link prediction in graphs is studied by modeling the dyadic interactions among two nodes. The relationships can be more complex than simple dyadic interactions and could require the user to model super-dyadic associations among nodes. Such interactions can be modeled using a hypergraph, which is a generalization of a graph where a hyperedge can connect more than two nodes. In this work, we consider the problem of hyperedge prediction in a $k-$uniform hypergraph. We utilize the tensor-based representation of hypergraphs and propose a novel interpretation of the tensor eigenvectors. This is further used to propose a hyperedge prediction algorithm. The proposed algorithm utilizes the \textit{Fiedler} eigenvector computed using tensor eigenvalue decomposition of hypergraph Laplacian. The \textit{Fiedler} eigenvector is used to evaluate the construction cost of new hyperedges, which is further utilized to determine the most probable hyperedges to be constructed. The functioning and efficacy of the proposed method are illustrated using some example hypergraphs and a few real datasets. The code for the proposed method is available on https://github.com/d-maurya/hypred_ tensorEVD

==> figs/hyred_sameGr.tex <==
\begin{tikzpicture}[scale = 0.6]
    \node (v1) at (0,2) {};
    \node (v2) at (2,2) {};
    \node (v3) at (0,0) {};
    \node (v4) at (2,0) {};
    
   
    \draw[] ($(v2) + (0.3,0)$) 
        to[out=270,in=90] ($(v4) + (0.3,0)$)
        to[out=270,in=0] ($(v4) + (0,-0.3)$)
        to[out=180,in=0] ($(v3) + (0,-0.3)$)
        to[out=180,in=270] ($(v3) + (-0.3,0)$)
        to[out=90,in=270] ($(v1) + (-0.3,0)$)
        to[out=90,in=180] ($(v1) + (0,0.3)$)
        to[out=0,in=180] ($(v2) + (0,0.3)$)
        to[out=0,in=90] ($(v2) + (0.3,0)$);
  
  \foreach \v in {1,2,...,4} {
        \fill (v\v) circle (0.1);
    }
    
   % \fill (v1) circle (0.1) node [above left =0.12cm] {$v_1$};
%    \fill (v2) circle (0.1) node [above right = 0.2cm] {$v_2$};
%    \fill (v3) circle (0.1) node [left = 0.3cm] {$v_3$};
%    \fill (v4) circle (0.1) node [below= 0.35cm] {$v_4$};
  
  % reduced graph 
    \node (r1) at (7,0) {};
    \node (r2) at (9,0) {};
    \node (r3) at (7,-2) {};
    \node (r4) at (9,-2) {};
    
    \foreach \v in {1,2,...,4} {
        \fill (r\v) circle (0.1);
    }
    
   % \fill (r1) circle (0.1) node [above left =0.12cm] {$v_1$};
%    \fill (r2) circle (0.1) node [above right = 0.2cm] {$v_2$};
%    \fill (r3) circle (0.1) node [left = 0.3cm] {$v_3$};
%    \fill (r4) circle (0.1) node [below= 0.35cm] {$v_4$};
    
    
   \draw[] ($(r1)$) to ($(r2)$);
   \draw[] ($(r1)$) to ($(r3)$);
   \draw[] ($(r1)$) to ($(r4)$);
   \draw[] ($(r2)$) to ($(r3)$);
   \draw[] ($(r2)$) to ($(r4)$);
   \draw[] ($(r3)$) to ($(r4)$);
   % reduced graph complete  
   
   % point the arrow for graph reduction 
   % arrow length
   % https://tex.stackexchange.com/questions/5461/is-it-possible-to-change-the-size-of-an-arrowhead-in-tikz-pgf/161238#161238
   \node (v5) at (2.3,1) {};
   \node (r5) at (6.8,-1) {};
  % \draw [|->, line width = 1 pt,dotted] (v5) edge (r5);
   \draw[-{Latex[length=5mm, width=2mm]}] (v5)--(r5);
   \draw[-{Latex[red,length=3mm, width=2mm]}] (9.1,-1)--(9.9,-1) node[right]{Represent G as Matrix};
   
   
   % draw another hypergraph 
    \node (g1) at (0,-2) {};
    \node (g2) at (2,-2) {};
    \node (g3) at (0,-4) {};
    \node (g4) at (2,-4) {};   
   
    
    \node (e1) at (1,-1.5) {\textcolor{red}{$\frac{1}{2}$}};
    \node (e1) at (2.5,-2.5) {\textcolor{black!30!cyan}{$\frac{1}{2}$}};
    \node (e1) at (1,-4.7) {\textcolor{black!50!pink}{$\frac{1}{2}$}};
    \node (e1) at (-0.7,-3) {\textcolor{black!30!green}{$\frac{1}{2}$}};
   % \node (e1) at (-1,0.05) {\textcolor{blue}{$e_2$}};
%    \node (e1) at (1,-0.75) {\textcolor{red}{$e_3$}};
    
     \draw[black!30!green] ($(g1)+(-0.2,0)$) 
        to[out=270,in=90] ($(g3) + (-0.2,0)$) 
        to[out=270,in=180] ($(g3) + (0,-0.2)$)
        to[out=0,in=270] ($(g3) + (0.2,0)$)
        to[out=90,in=270] ($(g1) + (0.2,-0.2)$)
        to[out=0,in=180] ($(g2) + (0,-0.2)$)
        to[out=0,in=270] ($(g2) + (0.2,0)$)
        to[out=90,in=0] ($(g2) + (0,0.2)$) 
        to[out=180,in=0] ($(g1) + (0,0.2)$)
        to[out=180,in=90] ($(g1) + (-0.2,0)$) ; 

    
    \draw[red] ($(g1)+(0,-0.15)$) 
        to[out=0,in=180] ($(g2) + (-0.1,-0.15)$) 
        to[out=270,in=90] ($(g4) + (-0.15,0)$)
        to[out=270,in=180] ($(g4) + (0,-0.15)$)
        to[out=0,in=270] ($(g4) + (0.15,0)$)
        to[out=90,in=270] ($(g2) + (0.15,0)$)
        to[out=90,in=0] ($(g2) + (0,0.15)$)
        to[out=180,in=0] ($(g1) + (0,0.15)$)
        to[out=180,in=90] ($(g1) + (-0.15,0)$)
        to[out=270,in=180] ($(g1) + (0,-0.15)$);
    
    \draw[black!30!cyan] ($(g2) + (0.3,0)$) 
        to[out=270,in=90] ($(g4) + (0.3,0)$)
        to[out=270,in=0] ($(g4) + (0,-0.3)$)
        to[out=180,in=0] ($(g3) + (0,-0.3)$)
        to[out=180,in=270] ($(g3) + (-0.3,0)$)
        to[out=90,in=180] ($(g3) + (0,0.3)$)
        to[out=0,in=180] ($(g4) + (-0.3,0.3)$)
        to[out=90,in=270] ($(g2) + (-0.3,0)$)
        to[out=90,in=180] ($(g2) + (0,0.3)$)
        to[out=0,in=90] ($(g2) + (0.3,0)$);
    
    \draw[black!50!pink] ($(g4) + (0.4,0)$)
        to[out=270,in=0] ($(g4) + (0,-0.4)$)
        to[out=180,in=0] ($(g3) + (0,-0.4)$)
        to[out=180,in=270] ($(g3) + (-0.4,0)$)
        to[out=90,in=270] ($(g1) + (-0.4,0)$)
        to[out=90,in=180] ($(g1) + (0,0.4)$)
        to[out=0,in=90] ($(g1) + (0.4,0)$)
        to[out=270,in=90] ($(g3) + (0.4,0.4)$)
        to[out=0,in=180] ($(g4) + (0,0.4)$)
        to[out=0,in=90] ($(g4) + (0.4,0)$);
    
        
  %  \fill (g1) circle (0.1) node [above left =0.12cm] {$v_1$};
  %  \fill (g2) circle (0.1) node [above right = 0.2cm] {$v_2$};
  %  \fill (g3) circle (0.1) node [left = 0.3cm] {$v_3$};
  %  \fill (g4) circle (0.1) node [below= 0.35cm] {$v_4$};
    
    
    \node (g5) at (2.3,-3) {};
  % \node (r6) at (6.8,-1) {};
  % \draw [|->, line width = 1 pt,dotted] (v5) edge (r5);
   \draw[-{Latex[length=5mm, width=2mm]}] (g5)--(r5);
    
\end{tikzpicture} 


==> synth_hy/ex2.tex <==
\subsection{Example 2} 
In the previous example, the performance of the proposed algorithm was justified using the basic properties of hypergraphs. In this example, we remove one of the hyperedges from the hypergraph H5 shown in Figure \ref{fig:ex2_3uni} to get H6 as shown in Figure \ref{fig:ex2_3uni_onedel} and investigate if the proposed algorithm is capable of predicting it. 

\begin{figure}[H]
	\centering
\begin{tikzpicture}
    \node (v1) at (0,2) {};
    \node (v2) at (2,2) {};
    \node (v3) at (0,0) {};
    \node (v4) at (2,0) {};
    \node (v5) at (3,1) {};
    \node (v6) at (4,2) {};
    \node (v7) at (4,0) {};
    \node (v8) at (6,0) {};
    \node (v9) at (6,2) {};
    
% draw hyperedges 
    \begin{scope}[fill opacity=0.8]

    \draw[fill = yellow!70] ($(v1)+(-0.3,0)$) 
        to[out=270,in=90] ($(v3) + (-0.3,0)$) 
        to[out=270,in=180] ($(v3) + (0,-0.3)$)
        to[out=0,in=270] ($(v3) + (0.3,0)$)
        to[out=90,in=270] ($(v1) + (0.3,-0.3)$)
        to[out=0,in=180] ($(v2) + (0,-0.3)$)
        to[out=0,in=270] ($(v2) + (0.3,0)$)
        to[out=90,in=0] ($(v2) + (0,0.3)$) 
        to[out=180,in=0] ($(v1) + (0,0.3)$)
        to[out=180,in=90] ($(v1) + (-0.3,0)$) ; 

%        to[out=180,in=270] ($(v1) + (-0.6,0.3)$);
%        to[out=120,in=250] ($(v1) + (-0.3,0.2)$);
    \draw[fill = red!100] ($(v6)+(0,-0.2)$) 
        to[out=0,in=180] ($(v9) + (-0.2,-0.2)$) 
        to[out=270,in=90] ($(v8) + (-0.2,0)$)
        to[out=270,in=180] ($(v8) + (0,-0.2)$)
        to[out=0,in=270] ($(v8) + (0.2,0)$)
        to[out=90,in=270] ($(v9) + (0.2,0)$)
        to[out=90,in=0] ($(v9) + (0,0.2)$)
        to[out=180,in=0] ($(v6) + (0,0.2)$)
        to[out=180,in=90] ($(v6) + (-0.2,0)$)
        to[out=270,in=180] ($(v6) + (0,-0.2)$);
    
    \draw[fill = red!100] ($(v1)+(0,-0.2)$) 
        to[out=0,in=180] ($(v2) + (-0.2,-0.2)$) 
        to[out=270,in=90] ($(v4) + (-0.2,0)$)
        to[out=270,in=180] ($(v4) + (0,-0.2)$)
        to[out=0,in=270] ($(v4) + (0.2,0)$)
        to[out=90,in=270] ($(v2) + (0.2,0)$)
        to[out=90,in=0] ($(v2) + (0,0.2)$)
        to[out=180,in=0] ($(v1) + (0,0.2)$)
        to[out=180,in=90] ($(v1) + (-0.2,0)$)
        to[out=270,in=180] ($(v1) + (0,-0.2)$);
        
    \draw[fill = cyan!70] ($(v2) + (0.4,0)$) 
        to[out=270,in=90] ($(v4) + (0.4,0)$)
        to[out=270,in=0] ($(v4) + (0,-0.4)$)
        to[out=180,in=0] ($(v3) + (0,-0.4)$)
        to[out=180,in=270] ($(v3) + (-0.4,0)$)
        to[out=90,in=180] ($(v3) + (0,0.4)$)
        to[out=0,in=180] ($(v4) + (-0.4,0.4)$)
        to[out=90,in=90] ($(v2) + (-0.4,0)$)
        to[out=90,in=180] ($(v2) + (0,0.4)$)
        to[out=0,in=90] ($(v2) + (0.4,0)$);
    
    
        
    \draw[fill = green!100] ($(v4)+(-0.3,0)$) 
        to[out=45,in=225] ($(v6) + (-0.3,0)$) % [out=alpha,in=beta], means alpha angle out from v4 (previous) node and beta angle in at the node v6 (or next node)  
      %  to[out=250,in=30] ($(v4)+(-0.2,-0.2)$)  
    to[out=45,in=90] ($(v6) + (0.3,0)$) 
    to[out=225,in=45] ($(v4) + (0.3,0)$) 
    to[out=250,in=225] ($(v4) + (-0.3,0)$);
    
        
    \draw[fill = cyan!70] ($(v6) + (-0.25,0)$) 
        to[out=270,in=90] ($(v7) + (-0.25,0)$) 
        to[out=270,in=180] ($(v7) + (0,-0.25)$) 
        to[out=0,in=180] ($(v8) + (0,-0.25)$)
        to[out=0,in=270] ($(v8) + (0.25,0)$)
        to[out=90,in=0] ($(v8) + (0,0.25)$)
        to[out=180,in=0] ($(v7) + (0.25,0.25)$)
        to[out=90,in=270] ($(v6) + (0.25,0)$)
        to[out=90,in=0] ($(v6) + (0,0.25)$)
        to[out=180,in=90] ($(v6) + (-0.25,0)$);
%        to[out=90,in=180] ($(v9) + (-0.15,0.25)$)
%        to[out=180,in=0] ($(v9) + (0.45,0.25)$);

    \end{scope}

% node symbol 
    \foreach \v in {1,2,...,9} {
        \fill (v\v) circle (0.1);
    }

% node names 
    \fill (v1) circle (0.1) node [above left =0.12cm] {$v_1$};
    \fill (v2) circle (0.1) node [above right = 0.2cm] {$v_2$};
    \fill (v3) circle (0.1) node [left = 0.3cm] {$v_3$};
    \fill (v4) circle (0.1) node [below= 0.35cm] {$v_4$};
    \fill (v5) circle (0.1) node [below right] {$v_5$};
    \fill (v6) circle (0.1) node [above = 0.3cm] {$v_6$};
    \fill (v7) circle (0.1) node [below= 0.33cm] {$v_7$};
    \fill (v8) circle (0.1) node [below = 0.33cm] {$v_8$};
    \fill (v9) circle (0.1) node [above = 0.3cm] {$v_9$};

% edge names using node(latex wala)
\end{tikzpicture}
	\caption{H6: Hyperedge $\{7,8,9\}$ removed from H5}
	\label{fig:ex2_3uni_onedel}
\end{figure}

%The new hypergraph after removal of hyperedge $\{7,8,9\}$ is shown in Figure (ref). 
The proposed algorithm mentioned in Table \ref{tab:algo} is applied, and the preferential order of potential hyperedges using unnormalized and normalized Laplacian is mentioned in Table \ref{tab:ex2_hypa}.  

\begin{table}[H]
  \caption{Preferential order of new hyperedges using unnormalized and normalized tensor Laplacian}
  \label{tab:ex2_hypa}
  \begin{center}
  \begin{tabular}{c|c}
    \toprule
    Unnormalized  & Normalized \\
    \midrule
    $\{1,3 ,    4\}$ &    $\{ 1   ,  3    , 4\}$ \\
    $\{7,8 ,    9\}$ &     $\{7   ,  8    , 9\}$\\
    $\{2,4 ,    5\}$ &     $\{5   ,  8    , 9\}$\\
    $\{1,     4     ,5\}$ &  $\{   5    , 6,     9\}$\\
    $\{3 ,    4     ,5\}$ & $\{    5    , 6     ,8\}$\\
    $\{5  ,   6     ,9\}$ &   $\{  5    , 7    , 8\}$\\
    $\{1  ,   2    , 5\}$ &     $\{5    , 7   ,  9\}$\\
    $\{2   ,  3   ,  5\}$ &     $\{6    , 7  ,   9\}$\\
    $\{1  ,   3 ,    5\}$ &     $\{1    , 5 ,    6\}$\\
    $\{5  ,   8  ,   9\}$ & $\{    3    , 5 ,    6\}$\\
  \bottomrule
\end{tabular}
 \end{center}
\end{table}

It can be observed that both the cases report the same. 
%(XZ top-2?) 
First two most preferred hyperedges. The hyperedges $ \{1,3, 4\}$ is the most preferred hyperedge because it has the most densely connected nodes, but it should be noticed that the second most preferred hyperedge is   $ \{7,8, 9\}$ which was removed in the beginning. 

It should also be noted that there is a slight change in the preferential order of the potential hyperedges if the hyperedge $ \{7,8, 9\}$ is removed. It may be concluded that the desired hyperedge is predicted with preferential order of 2 as it is the second most preferred hyperedge among $78$ potential hyperedges. 

==> synth_hy/ex3.tex <==
\subsection{Example 3}

In the previous example, it was established that the proposed algorithm is capable of predicting the removed hyperedges. In this example, we study the performance of the algorithm in predicting hyperedges with different properties. For example, it is expected that any hyperedge prediction algorithm will most probably predict a  hyperedge with nodes which are densely connected with other nodes. 
% (XZ : Relevance of the example and the property is not clear)

\begin{figure}[H]
	\centering
	\includegraphics[width=0.72\linewidth]{figs/uni3_2cl.png}
	\caption{3-uniform hypergraph for Example 3}
	\label{fig:ex3_3uni_2cl}
\end{figure}

Consider the 3-uniform hypergraph presented in Figure \ref{fig:ex3_3uni_2cl}. It consists of 12 nodes and nine hyperedges. We remove each of the hyperedges one at a time and compute its preferential order among all the $212$ potential hyperedges. The preferential order is computed using unnormalized ($po_u$) and  normalized ($po_n$) version of Laplacian tensor and is summarized in Table \ref{tab:ex3_ran}. 

\begin{table}[H]
  \caption{Preferntial Order using unnormalized and normalized Laplacian tensor}
  \label{tab:ex3_ran}
  \begin{center}
  \begin{tabular}{c|c|c}
    \toprule
    Deleted hyperedge & $po_u$ &$ po_n$ \\
    \midrule
    $\{1,2,3\}$ & 80 & 26\\
    $\{2,3,4\}$& 41  & 30 \\
    $\{3,4,5\}$ & 82 & 59 \\
    $\{1,5,6\}$ & 97 & 45 \\
    $\{6,7,8\}$ & 110 & 52 \\
    $\{7,9,10\}$ & 207 & 204\\
    $\{9,10,11\}$ & 146 & 113\\
    $\{10,11,12\}$ & 148 & 111\\
    $\{11,12,8\}$ & 206 & 204\\    
    \bottomrule
\end{tabular}
\end{center}
\end{table}
We can interpret the Table \ref{tab:ex3_ran} as follows. Consider the hyperedge $\{1,2,3\}$ with a preferential order of $26$ using the normalized Laplacian tensor. This states that there were 25 other hyperedges which were more likely to be formed if the hyperedge $\{1,2,3\}$ is removed. It should be noted that this preferential order is ranked among all $213$ potential hyperedges.  

Ideally, a lower preferential order is desired. It can be observed that the analysis of normalized tensor Laplacian establishes better preferential order. 
% (XZ: Point seems disconnected. Tarun, please re-write)

% Several other interesting questions can be answered using the hyperedge construction cost presented in Table \ref{tab:ex1_cost_unnorm} and Table \ref{tab:ex1_cost_norm}(XZ The hyperedge construction cost presented in Table \ref{tab:ex1_cost_unnorm} opens up new avenues for several interesting questions). For example, we can answer which is most probable hyperedge given node 2 and 5 should be present in that hyperedge? The most preferable third node will be $4$ as it has minimum construction cost shown in Table  \ref{tab:ex1_cost_unnorm}. (XZ Change this. Looks very juvenile)

% These questions find interesting applications in co-author networks where two authors are known and searching for the best choice of third collaborator.
The hyperedge construction cost presented in Table \ref{tab:ex3_ran} opens up new avenues for several interesting questions. Consider the problem of estimating the preferential order given a few nodes in a hyperedge. For example, we can predict the preferable third node given the presence of two nodes after the removal of hyperedge $\{1,2,3\}$. As the two nodes in a hyperedge are known, the number of potential hyperedges reduces from 213 to 10 (as there are 12 nodes and 2 are assumed to be known in a new hyperedge). 
\begin{table}[H]
  \caption{Preferential Order of $3^{rd}$ node in $\{1,2,3\}$ given two nodes}
  \label{tab:ex3_given2}
  \begin{center}
  \begin{tabular}{c|c|c}
    \toprule
    Given Nodes & desired node & $ po_n$ \\
    \midrule
    $\{1,2\}$ & 3 & 1\\
    $\{1,3\}$&  2 & 3 \\
    $\{2,3\}$ & 1 & 1 \\
    \bottomrule
\end{tabular}
\end{center}
\end{table}
The table \ref{tab:ex3_given2} contains the preferential order for the third node given the other two nodes.
It can be observed that the preferential order has significantly improved if partial information about the potential hyperedge is passed as an input to the proposed algorithm. 

This observation manifests that such interesting questions can be easily addressed using the proposed algorithm. 

==> synth_hy/ex4.tex <==
\subsection{Example 4}
In the previous examples, we have considered $3$-uniform hypergraphs only. As the algorithm is proposed for any k-uniform hypergraph, we now study the functioning of the algorithm on a 4-uniform hypergraph. 

Consider a 4-uniform hypergraph with nine nodes and five hyperedges shown in Figure \ref{fig:ex4}. We are assigned with the same task of hyperedge prediction for this given hypergraph. The same procedure is repeated, and we report the top 10 of the 205 potential hyperedges in Table \ref{tab:ex4_hyp} using the unnormalized and normalized Laplacian tensor. 

\begin{figure}[H]
	\centering
	\includegraphics[width=0.82\linewidth]{figs/uni4_.png}
	\caption{4-uniform hypergraph for Example 4}
	\label{fig:ex4}
\end{figure}



\begin{table}[H]
  \caption{Preferential order of new hyperedges using unnormalized and normalized tensor Laplacian}
  \label{tab:ex4_hyp}
  \begin{center}
  \begin{tabular}{c|c}
    \toprule
    Unnormalized  & Normalized \\
    \midrule
    $\{1,2, 3,9\}$ &  $\{2,5 ,6  , 9 \}$  \\  
       $\{  1,2,4,9 \}$ &   $\{1     ,  2 , 3 , 9 \}$ \\
    $\{  2,3,4,9 \}$ &      $\{1 ,2,4,9 \}  $\\
    $\{  5,7,8,10\}$ &  $\{     1,2, 5 , 9\} $ \\      
    $\{   5,6,8,10 \}$ & $\{   1,   2  , 6 ,  9\}  $ \\  
   $\{   1,3,4,5  \}$ & $\{ 5,  7,  8 , 10 \}   $ \\   
   $\{   2,3,4,5 \}$ &       $\{2, 3, 4, 9\}$ \\   
    $\{   3,4,5,9 \}$ &    $\{1,5    ,6,9\}  $ \\    
    $\{   1,2,4,5 \}$ & $\{ 1    , 2,  5    ,  6\} $  \\    
   $\{   1,3,5,9      \}$ & $\{ 2    , 3    , 5    ,  9\}$  \\ 
  \bottomrule
\end{tabular}
\end{center}
\end{table}
We draw similar observations regarding the formation of most probable hyperedges from Table \ref{tab:ex4_hyp}. We can also observe that the normalized Laplacian attempts to grant similar weight to all the nodes by normalizing with the degree of the node.   

In this section, we demonstrated the performance of the proposed algorithm using simple hypergraphs. Several interesting properties like detection of structurally similar hyperedges, behavior for unnormalized and normalized Laplacian tensor, behavior when partial information is supplied as input were investigated. 

All these inferences cannot be performed using by modeling dyadic interactions using matrix representation or hypergraph reduction methods. In the next section, we make concluding remarks. 

